Fast-MbyM: Leveraging Translational Invariance of the Fourier Transform for Efficient and Accurate Radar Odometry

Masking By Moving (MByM), provides robust and accurate radar odometry measurements through an exhaustive correlative search across discretised pose candidates. However, this dense search creates a significant computational bottleneck which hinders real-time performance when high-end GPUs are not available. Utilising the translational invariance of the Fourier Transform, in our approach, f-MByM, we decouple the search for angle and translation. By maintaining end-to-end differentiability a neural network is used to mask scans and trained by supervising pose prediction directly. Training faster and with less memory, utilising a decoupled search allows f-MByM to achieve significant run-time performance improvements on a CPU (168%) and to run in real-time on embedded devices, in stark contrast to MByM. Throughout, our approach remains accurate and competitive with the best radar odometry variants available in the literature -- achieving an end-point drift of 2.01% in translation and 6.3deg/km on the Oxford Radar RobotCar Dataset.

==> 2-related-work.tex <==
\section{Related Work}
\label{sec:RelatedWorks}

With the exception of the work by Park \textit{et al}~\cite{park2020pharao}, the \emph{non-learned} family of techniques applied to \gls{ro} unerringly turns to stable feature extraction in order to deal with this complex scan formation process.
This includes the work of Cen and Newman~\cite{cen2018precise} on shape similarity metrics to remove outliers which was then improved in~\cite{cen2019radar} by a gradient-based feature detector and a new graph matching strategy.
Kung \textit{et al}~\cite{kung2021normal} use a \gls{ndt} typically applied to both 2D and 3D lidar.
Adolfsson \textit{et al}~\cite{adolfsson2021cfear} employ filtering to retain the strongest azimuthal returns and compute a sparse set of oriented surface points.
In~\cite{burnett2021we}, Burnett \textit{et al} use continuous-time estimation to compensate for motion distortion and Doppler effects.
Hong \textit{et al} \cite{hong2020radarslam} use vision-based features and graph-matching to achieve SLAM.

Further to this trend, some later variants are designed for \emph{learned} stable feature extraction or learning preprocessing operations for greater stability.
For example, in~\cite{barnes2020under}, Barnes and Posner use deep keypoint detectors and descriptors and differentiable point matching and pose estimation.
In~\cite{burnett2021radar}, Burnett \textit{et al} develop probabilistic trajectory estimation and unsupervised deep feature learning techniques.
Drawing on the strengths of both \emph{learned} and \emph{non-learned} techniques, Aldera \textit{et al}~\cite{aldera2019fast} build on the classical feature system of~\cite{cen2018precise} and train a focus of attention network to downsample measurements for more rapid data association, while in~\cite{aldera2019could} a linear classifier is learned to diagnose and filter erroneous motion estimates.\gadd{oRO reference}

In contrast to these sparse variants, the greatest \gls{ro} performance in terms of accuracy seems to be achieved by dense registration techniques which are stabilised by preprocessing, all operations being \emph{learned} in an end-to-end fashion from vast data.
Here, the state-of-the-art, \gls{mbym} by Barnes \textit{et al}~\cite{barnes2019masking}, uses a correlation-based approach with learned masking to ignore moving objects and noise artefacts.
It is, however, as mentioned in~\cref{sec:Introduction}, not readily deployable to mobile machines with reasonable compute resources.

In the area of dense registration techniques, Fourier analysis as employed by Barnes \textit{et al}~\cite{barnes2019masking} is under various log-polar transformations useful for recovering rotational, translational, and scaling differences between similar views~\cite{lim1990two}.
Indeed, it has been applied to \gls{vo} in~\cite{kazik2011visual,ho2008optical}, drawing on early image registration work by Casasent and Psaltis~\cite{casasent1976position}.
Kazik and G{\"o}kto{\u{g}}an~\cite{kazik2011visual} use a single ground-facing camera, necessitating the scale-aware \gls{fmt} due to the lack of depth constraints in the monocular setup, showing better performance than optical flow formulations such as by Ho and Goecke~\cite{ho2008optical}.

In the radar domain, Park \textit{et al}~\cite{park2020pharao} apply the \gls{fmt} to log-polar images computed from downsampled Cartesian images.
This draws on the \gls{fmt} formulation of radar scan matching by Checchin and G{\'e}rossier~\cite{checchin2010radar} which is included within an \acrshort{ekf} \acrshort{slam} system.
In these \gls{fmt} formulations, the \gls{ft} of the input images are remapped to log-polar coordinates and rotation and scaling is expressed as translations in the resulting image.
As in~\cite{barnes2019masking}, these parameters are in fact recoverable using the native \gls{ft}.
However, the \gls{fmt} is designed for efficiency in recovering rotation.

Nevertheless, in this work we recognise that the \gls{fmt} accounts for scale change -- this integral transform is unnecessary in the radar domain -- and that the affine transformation property of the \gls{ft} allows for pose estimation to be separated into a two-step rotation-then-translation procedure.
We therefore present a system which in contrast with~\cite{park2020pharao} exploits learning of a stabilising masking function for greater accuracy and in contrast with~\cite{barnes2019masking} can run on realistic processing platforms.


==> plots/ablation.tex <==
\pgfplotsset{
select row/.style={
x filter/.code={\ifnum\coordindex=#1\else\def\pgfmathresult{}\fi}
}
}

\definecolor{ao}{rgb}{0.0, 0.5, 0.0}

\pgfplotstableread[col sep=comma]{
nlvls,TP,JS
3,0.03618848324,0.115851223
4,0.03920197487,0.1191828918
5,0.0430765152,0.1221413536
6,0.04613244534,0.1255276566
}\nlvlsData

\pgfplotstableread[col sep=comma]{
nlvls,tr
3,4.044916522
4,2.839134474
5,2.712216522
6,2.266691908
}\nlvlsTrData

\pgfplotstableread[col sep=comma]{
nlvls,ro
3,0.01269764511
4,0.01005850649
5,0.008704939645
6,0.007224818371
}\nlvlsRoData

\pgfplotstableread[col sep=comma]{
nxy,TP,JS
125,0.01985013485,0.05330432129
155,0.02597844601,0.06770166397
185,0.03350555897,0.08216732025
215,0.03480744362,0.1005846901
255,0.04832732677,0.1285452881
285,0.05754339695,0.1630497665
}\nxyData

\pgfplotstableread[col sep=comma]{
nxy,tr
125,2.597204926
155,2.722349904
185,1.821482344
215,2.158546799
255,1.70952555
}\nxyTrData

\pgfplotstableread[col sep=comma]{
nxy,ro
125,0.008399707913
155,0.009101650196
185,0.005798968829
215,0.007144045183
255,0.005515250613
}\nxyRoData

\begin{figure*}[h]
\centering
%
\subfloat[]{
{\scalefont{0.5}
\begin{tikzpicture}
\begin{axis}[
ybar,
bar width=.15cm,
width=5cm,
height=2.8cm,
enlarge x limits=0.15,
% legend style={at={(0.5,1.2)}, anchor=north,legend columns=-1},
symbolic x coords = {3,4,5,6},
xtick=data,
xlabel={$\mathrm{nlvls}$},
ylabel={$f~[\SI{}{\hertz}]$},
x label style={at={(axis description cs:1,0.15)},rotate=0,anchor=south},
y label style={at={(axis description cs:0.5,1.2)},rotate=-90,anchor=north},
yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=5},
scaled y ticks=false,
grid=major,
xmajorgrids=false
]
\addplot[blue!20!blue,fill=blue!80!white] table[x=nlvls,y expr=1.0/\thisrow{TP}]{\nlvlsData};
% \addplot[red!20!red,fill=red!80!white] table[x=nlvls,y expr=1.0/\thisrow{JS}]{\nlvlsData};
% \legend{\texttt{TP},\texttt{JS}}
\end{axis}
\end{tikzpicture}
}
}
%
\subfloat[]{
{\scalefont{0.5}
\begin{tikzpicture}
\begin{axis}[
ybar,
bar width=.15cm,
width=5cm,
height=2.8cm,
enlarge x limits=0.15,
% legend style={at={(0.5,1.2)}, anchor=north,legend columns=-1},
symbolic x coords = {3,4,5,6},
xtick=data,
xlabel={$\mathrm{nlvls}$},
ylabel={$f~[\SI{}{\hertz}]$},
x label style={at={(axis description cs:1,0.15)},rotate=0,anchor=south},
y label style={at={(axis description cs:0.5,1.2)},rotate=-90,anchor=north},
yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=5},
scaled y ticks=false,
grid=major,
xmajorgrids=false
]
% \addplot[blue!20!blue,fill=blue!80!white] table[x=nlvls,y expr=1.0/\thisrow{TP}]{\nlvlsData};
\addplot[red!20!red,fill=red!80!white] table[x=nlvls,y expr=1.0/\thisrow{JS}]{\nlvlsData};
% \legend{\texttt{TP},\texttt{JS}}
\end{axis}
\end{tikzpicture}
}
}
%
\subfloat[]{
{\scalefont{0.5}
\begin{tikzpicture}
\begin{axis}[
ybar,
bar width=.15cm,
width=5cm,
height=2.8cm,
enlarge x limits=0.15,
% legend style={at={(0.4,1.3)}, anchor=north,legend columns=-1},
symbolic x coords = {125,155,185,215,255,285},
xtick=data,
xlabel={$\mathrm{nxy}$},
ylabel={$f~[\SI{}{\hertz}]$},
x label style={at={(axis description cs:1,0.15)},rotate=0,anchor=south},
y label style={at={(axis description cs:0.5,1.2)},rotate=-90,anchor=north},
yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=5},
scaled y ticks=false,
grid=major,
xmajorgrids=false
]
\addplot[blue!20!blue,fill=blue!80!white] table[x=nxy,y expr=1.0/\thisrow{TP}]{\nxyData};
% \addplot[red!20!red,fill=red!80!white] table[x=nxy,y expr=1.0/\thisrow{JS}]{\nxyData};
% \legend{\texttt{TP},\texttt{JS}}
\end{axis}
\end{tikzpicture}
}
}
%
\subfloat[]{
{\scalefont{0.5}
\begin{tikzpicture}
\begin{axis}[
ybar,
bar width=.15cm,
width=5cm,
height=2.8cm,
enlarge x limits=0.15,
% legend style={at={(0.4,1.3)}, anchor=north,legend columns=-1},
symbolic x coords = {125,155,185,215,255,285},
xtick=data,
xlabel={$\mathrm{nxy}$},
ylabel={$f~[\SI{}{\hertz}]$},
x label style={at={(axis description cs:1,0.15)},rotate=0,anchor=south},
y label style={at={(axis description cs:0.5,1.2)},rotate=-90,anchor=north},
yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=5},
scaled y ticks=false,
grid=major,
xmajorgrids=false
]
% \addplot[blue!20!blue,fill=blue!80!white] table[x=nxy,y expr=1.0/\thisrow{TP}]{\nxyData};
\addplot[red!20!red,fill=red!80!white] table[x=nxy,y expr=1.0/\thisrow{JS}]{\nxyData};
% \legend{\texttt{TP},\texttt{JS}}
\end{axis}
\end{tikzpicture}
}
}

\subfloat[]{
{\scalefont{0.5}
\begin{tikzpicture}
\begin{axis}[
ybar,
bar width=.15cm,
width=5cm,
height=2.8cm,
enlarge x limits=0.15,
% legend style={at={(0.6,0.9)}, anchor=north,legend columns=-1},
symbolic x coords = {3,4,5,6},
xtick=data,
xlabel={$\mathrm{nlvls}$},
ylabel={$\mathrm{Tr}~[\SI{}{\percent}]$},
x label style={at={(axis description cs:1,0.15)},rotate=0,anchor=south},
y label style={at={(axis description cs:0.75,1.2)},rotate=-90,anchor=north},
yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=5},
scaled y ticks=false,
grid=major,
xmajorgrids=false
]
\addplot[ao!20!ao,fill=ao!80!white] table[x=nlvls,y=tr]{\nlvlsTrData};
% \addplot[orange!20!orange,fill=orange!80!white] table[x=nlvls,y expr=\thisrow{ro}*100]{\nlvlsRoData};
% \legend{\texttt{Tr},\texttt{Ro}}
\end{axis}
\end{tikzpicture}
}
}
%
\subfloat[]{
{\scalefont{0.5}
\begin{tikzpicture}
\begin{axis}[
ybar,
bar width=.15cm,
width=5cm,
height=2.8cm,
enlarge x limits=0.15,
% legend style={at={(0.6,0.9)}, anchor=north,legend columns=-1},
symbolic x coords = {3,4,5,6},
xtick=data,
xlabel={$\mathrm{nlvls}$},
ylabel={$\mathrm{Ro}~[\SI{}{\deg\per\kilo\metre}]$},
x label style={at={(axis description cs:1,0.15)},rotate=0,anchor=south},
y label style={at={(axis description cs:0.75,1.2)},rotate=-90,anchor=north},
yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=5},
scaled y ticks=false,
grid=major,
xmajorgrids=false
]
% \addplot[ao!20!ao,fill=ao!80!white] table[x=nlvls,y=tr]{\nlvlsTrData};
\addplot[orange!20!orange,fill=orange!80!white] table[x=nlvls,y expr=\thisrow{ro}*1000]{\nlvlsRoData};
% \legend{\texttt{Tr},\texttt{Ro}}
\end{axis}
\end{tikzpicture}
}
}
%
\subfloat[]{
{\scalefont{0.5}
\begin{tikzpicture}
\begin{axis}[
ybar,
bar width=.15cm,
width=5cm,
height=2.8cm,
enlarge x limits=0.15,
% legend style={at={(0.5,1.2)}, anchor=north,legend columns=-1},
symbolic x coords = {125,155,185,215,255,285},
xtick=data,
xlabel={$\mathrm{nxy}$},
ylabel={$\mathrm{Tr}~[\SI{}{\percent}]$},
x label style={at={(axis description cs:1,0.15)},rotate=0,anchor=south},
y label style={at={(axis description cs:0.75,1.2)},rotate=-90,anchor=north},
yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=5},
scaled y ticks=false,
grid=major,
xmajorgrids=false
]
\addplot[ao!20!ao,fill=ao!80!white] table[x=nxy,y=tr]{\nxyTrData};
% \addplot[orange!20!orange,fill=orange!80!white] table[x=nxy,y expr=\thisrow{ro}*100]{\nxyRoData};
% \legend{\texttt{Tr},\texttt{Ro}}
\end{axis}
\end{tikzpicture}
}
}
%
\subfloat[]{
{\scalefont{0.5}
\begin{tikzpicture}
\begin{axis}[
ybar,
bar width=.15cm,
width=5cm,
height=2.8cm,
enlarge x limits=0.15,
% legend style={at={(0.5,1.2)}, anchor=north,legend columns=-1},
symbolic x coords = {125,155,185,215,255,285},
xtick=data,
xlabel={$\mathrm{nxy}$},
ylabel={$\mathrm{Ro}~[\SI{}{\deg\per\kilo\metre}]$},
x label style={at={(axis description cs:1,0.15)},rotate=0,anchor=south},
y label style={at={(axis description cs:0.75,1.2)},rotate=-90,anchor=north},
yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=3},
scaled y ticks=false,
grid=major,
xmajorgrids=false
]
% \addplot[ao!20!ao,fill=ao!80!white] table[x=nxy,y=tr]{\nxyTrData};
\addplot[orange!20!orange,fill=orange!80!white] table[x=nxy,y expr=\thisrow{ro}*1000]{\nxyRoData};
% \legend{\texttt{Tr},\texttt{Ro}}
\end{axis}
\end{tikzpicture}
}
}
%
\caption{
Ablation study, effect of removing layers on the real-time performance of our system.
\gadd{some numbers are wrong?}
\gadd{Tr/Ro in text}
\gadd{axes labels pos}
\gadd{colors}
\gadd{bottom row shifted}
\gadd{discuss in text}
}
\label{fig:ablation}
\end{figure*}

